SurvRNC: Learning Ordered Representations for Survival Prediction using Rank-N-Contrast

Predicting the likelihood of survival is of paramount importance for individuals diagnosed with cancer as it provides invaluable information regarding prognosis at an early stage. This knowledge enables the formulation of effective treatment plans that lead to improved patient outcomes. In the past few years, deep learning models have provided a feasible solution for assessing medical images, electronic health records, and genomic data to estimate cancer risk scores. However, these models often fall short of their potential because they struggle to learn regression-aware feature representations. In this study, we propose Survival Rank-N Contrast (SurvRNC) method, which introduces a loss function as a regularizer to obtain an ordered representation based on the survival times. This function can handle censored data and can be incorporated into any survival model to ensure that the learned representation is ordinal. The model was extensively evaluated on a HEad \& NeCK TumOR (HECKTOR) segmentation and the outcome-prediction task dataset. We demonstrate that using the SurvRNC method for training can achieve higher performance on different deep survival models. Additionally, it outperforms state-of-the-art methods by 3.6% on the concordance index. The code is publicly available on https://github.com/numanai/SurvRNC

==> tables/soa_abl.tex <==
\begin{table}
\centering

\begin{minipage}{0.45\textwidth}


%%%%%%%%%%%%%% Table: AFA (impact of quantization threshold, with ssim loss) %%%%%%%%%%%%%%
\caption{Ablation study for $\lambda$ values}
% \caption{\small{AFA ($\mathrm{steps}=20,~\mathrm{PatchSize}=(8\times 8 \times 8)$). (UNETR).}}
\label{tbl:afa-qmax-nossim-ssim}
\scalebox{0.8}{
\begin{tabular}{ l | c  c } 
\toprule
  \rowcolor{Gray}
  $\lambda$ & $\mathrm{0.3}\hspace{-0.3em}$ & $\mathrm{0.5}\hspace{-0.3em}$ \\
  \midrule
   % ~-   & \textcolor{OliveGreen}{74.31} & -  \\
   10   & 65.95 & \textbf{99.10} \\ 
   20   & 56.24 & 98.70 \\ 
   \bottomrule
\end{tabular}
}
\end{minipage}


\begin{minipage}{0.45\textwidth}
%%%%%%%%%%%%%% Table: Comparison of voxel and freq. domain attacks %%%%%%%%%%%%%%
\caption{\small{Comparision with state-of-the-art survival prediction methods}}
\label{tbl:soa_models}
\scalebox{0.8}{
\begin{tabular}{ l c | c } 
\toprule
\rowcolor{Gray}
 \multicolumn{2}{c|}{Methods} & $\mathrm{\textbf{CI}}\hspace{-0.3em}\uparrow$ \\
\midrule
% ~~~-  & \textcolor{OliveGreen}{74.31} & - \\
 CoxPH    & Radiomics &  0.745\scriptsize±0.024 \\ 
 ICARE   & Radiomics &  0.765\scriptsize±0.019 \\ 
Ensemble \cite{saeed2021ensemble}
& CNN &  0.748\scriptsize±0.025 \\ 
 TMSS \cite{saeed2022tmss}    & ViT+CNN &  0.761\scriptsize±0.028 \\
DeepMTS [24]  & CNN  &  0.757\scriptsize±0.022 \\ 
 XSurv & Hybrid  & 0.782\scriptsize±0.018 \\
Radio-XSurv [XX] & Hybrid+Rad.  & 0.798\scriptsize±0.015 \\
 \hline
\rowcolor{lightskyblue}
 SurvRNC* & CNN  & 0.827\scriptsize±0.034 \\
 \bottomrule
\end{tabular}
}
\end{minipage}
% \hspace{1.1em}
\end{table}
